Cycle-Configuration: A Novel Graph-theoretic Descriptor Set for Molecular Inference

In this paper, we propose a novel family of descriptors of chemical graphs, named cycle-configuration (CC), that can be used in the standard "two-layered (2L) model" of mol-infer, a molecular inference framework based on mixed integer linear programming (MILP) and machine learning (ML). Proposed descriptors capture the notion of ortho/meta/para patterns that appear in aromatic rings, which has been impossible in the framework so far. Computational experiments show that, when the new descriptors are supplied, we can construct prediction functions of similar or better performance for all of the 27 tested chemical properties. We also provide an MILP formulation that asks for a chemical graph with desired properties under the 2L model with CC descriptors (2L+CC model). We show that a chemical graph with up to 50 non-hydrogen vertices can be inferred in a practical time.

==> Makefile <==
# Makefile

# suffixes.
.SUFFIXES: .c .o .tex .dvi .ps .pdf

# macros.
CC = gcc
CFLAGS = -O2 -Wall -lm
#CFLAGS = -O2 -Wall -lm -ggdb -lefence
DVIPS = dvips
DVIPDF = dvipdfmx -p a4
PSPDF = ps2pdf14
LATEX = platex --kanji=utf-8
PDFLATEX = pdflatex
BIBTEX = pbibtex
OBJS = null
RM = rm -f
TARGET = null

# cleaning rules.
clean:
	$(RM) *.o *~ \#*
paperclean:
	$(RM) *.o *~ \#* $(PAPER).bbl $(PAPER).blg $(PAPER).aux $(PAPER).idx $(PAPER).toc $(PAPER).lo*


# generation rules.
PAPER = cc_main
BIB = CC_ref
#
$(PAPER).pdf:    $(PAPER).tex cc_intro.tex cc_preliminary.tex cc_cycle_config.tex cc_milp.tex cc_experiments.tex cc_conc.tex appendix_2Lmodel.tex appendix_MILP.tex $(PAPER).bbl
	$(BIBTEX) $(PAPER)
	$(PDFLATEX) $(PAPER).tex
	$(PDFLATEX) $(PAPER).tex

# $(PAPER).pdf:    $(PAPER).tex $(PAPER).bbl
#	$(BIBTEX) $(PAPER)
#	$(PDFLATEX) $(PAPER).tex
#	$(PDFLATEX) $(PAPER).tex
#
$(PAPER).bbl:    $(BIB).bib
	$(LATEX) $(PAPER).tex
	$(BIBTEX) $(PAPER)



# suffix rules: "$@ is dependent on $<".
.c.o:
	$(CC) $(CFLAGS) -c $<
.tex.dvi: $<
	$(LATEX) $<
	$(LATEX) $<

.dvi.pdf: $<
	$(DVIPDF) $<

#.tex.pdf: $<
#	$(PDFLATEX) $<
#	$(PDFLATEX) $<


# dependencies.

